On the Limitations of Carbon-Aware Temporal and Spatial Workload Shifting in the Cloud

Cloud platforms have been focusing on reducing their carbon emissions by shifting workloads across time and locations to when and where low-carbon energy is available. Despite the prominence of this idea, prior work has only quantified the potential of spatiotemporal workload shifting in narrow settings, i.e., for specific workloads in select regions. In particular, there has been limited work on quantifying an upper bound on the ideal and practical benefits of carbon-aware spatiotemporal workload shifting for a wide range of cloud workloads. To address the problem, we conduct a detailed data-driven analysis to understand the benefits and limitations of carbon-aware spatiotemporal scheduling for cloud workloads. We utilize carbon intensity data from 123 regions, encompassing most major cloud sites, to analyze two broad classes of workloads -- batch and interactive -- and their various characteristics, e.g., job duration, deadlines, and SLOs. Our findings show that while spatiotemporal workload shifting can reduce workloads' carbon emissions, the practical upper bounds of these carbon reductions are currently limited and far from ideal. We also show that simple scheduling policies often yield most of these reductions, with more sophisticated techniques yielding little additional benefit. Notably, we also find that the benefit of carbon-aware workload scheduling relative to carbon-agnostic scheduling will decrease as the energy supply becomes "greener".

==> 5-camera-ready-spatial.tex <==
We first quantify the theoretical limits of the spatial workload migration by considering an ideal scenario where all regions have datacenters with infinite capacity and workloads may migrate to anywhere in the world. We then analyze realistic settings that affect the carbon savings from spatial shifting, e.g., constrained migration, datacenter capacity, and latency. Lastly, we discuss the system implications and whether sophisticated policies are required to optimize for carbon savings. 

\begin{figure*}[!t]
	\centering
	\begin{tabular}{ccc}
		\includegraphics[width=0.3\linewidth]{figs-eurosys24/spatial/utilization/one_migration_w_cap_99.pdf} &
		\includegraphics[width=0.3\linewidth]{figs-eurosys24/spatial/utilization/one_migration_w_cap_50.pdf} &
		\includegraphics[width=0.3\linewidth]{figs-eurosys24/spatial/global-idle-cap/global_idle_cap.pdf} \\
		(a) Infinite Capacity & (b) With 50\% Utilization per region & (c) Intensity and Idle Capacity
	\end{tabular}
	\vspace{-0.3cm}
	\caption{\emph{Global carbon savings relative to regions' idle capacity: As the idle capacity increases, the overall carbon savings increase.}}   
	\vspace{-0.5cm}
	\label{fig:spatial-cap-figs}
\end{figure*}


\subsection{Savings with Infinite Capacity}
\label{subsec:spatial-inf-cap}

In this setting, regions have infinite capacity and workloads can migrate to the greenest region to maximize carbon savings. In our trace, Sweden has the lowest annual average carbon intensity in the world at $\sim$16 \carbonunit.  
Figure~\ref{fig:spatial-cap-figs}(a) shows the global decreases in carbon when taken across all regions, as well decreases for various geographical regions, both calculated relative to the average global carbon intensity. Since all jobs migrate to Sweden, the global average carbon intensity drops by 96\%. Given the variations in average carbon intensity across different geographical regions, which are contingent on their respective energy mix, the extent of relative savings resulting from spatial migration also varies significantly.
For example, Europe is the greenest overall region in the world with an average carbon intensity of $\sim$280 \carbonunit. Thus, its average savings are only 86\%, which is significantly less than the global savings.  In contrast, Asia has the highest average carbon intensity for any geographical region in the world,$\sim$540 \carbonunit, and thus gets the highest savings from moving to Sweden at 151\%.
\vspace{-0.2cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaway.} In the ideal case with infinite datacenter capacity, spatial shifting to the world's greenest cloud regions can lead to 96\% average reduction in emissions. Notably, high intensity regions experience the most substantial benefits when transitioning to the greenest locations.}
\end{visionbox}

\subsection{Savings with Capacity Constrains}
\label{subsec:spatial-cap-constrained}

As the scenario where all datacenter regions possess an unbounded capacity is not feasible, we also aim to assess the potential savings under practical conditions by considering capacity constraints. This constraint reflects real-world limitations and allows us to gauge the disparity between theoretical savings and practical outcomes.
Figure~\ref{fig:spatial-cap-figs}(b) illustrates the carbon savings associated with spatial shifting when we make the assumption that all regions worldwide possess identical capacity and are currently operating at 50\% idle capacity.  To examine the upper bound of a capacity-constrained setting, we also want to maximize the carbon savings in this scenario. In pursuing this, the region with the highest carbon intensity would transfer its workloads to the region with the lowest carbon intensity. Subsequently, the region with the second-highest carbon intensity would relocate its tasks to the second-lowest carbon intensity location, and so forth. Figure~\ref{fig:spatial-cap-figs}(b) shows that with 50\% idle capacity operations, the global carbon savings gained from spatial migration decrease to $\sim$52\% as compared to $\sim$96\% when there is no capacity constrained. Of particular interest is the fact that the spatial savings in Asia remains at 151\%. This illustrates the significant proportion of regions with high carbon intensity located in Asia, and relocating workloads from these regions yields substantial spatial savings.

Lastly, Figure~\ref{fig:spatial-cap-figs}(c) shows emission rates (in \emissionunit) as the global idle capacity increases. We assume uniform resources across all regions worldwide, and the idle capacity refers to the available capacity within each region for accommodating new workloads.
In the most extreme scenario, with idle capacity reaching 99\%, the greenest region has the capability to absorb all workloads from other regions.
As a result, the emission rate is $\sim$16 \emissionunit, which reflects the carbon intensity of Sweden -- the greenest region in our data set. Conversely, when the global idle capacity reaches 0\%, the emission rate levels off at 368.39 \emissionunit, representing the global average carbon intensity. In this scenario, no workloads can be relocated to other regions, resulting in each region solely managing its own workload. Increasing idle capacity by 99\% reduces the emission rate by $\sim$96\%, and in the less extreme case, increasing the global idle capacity to 50\% reduces the emission rate by 52\%. While increasing idle capacity helps regions to increase savings from spatial workload migration, the originating datacenters remain underutilized, which increases operational and non-operational costs such as embodied carbon. 

\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaway.}  In the practical case where datacenter capacity is finite, the savings from spatial shifting depend on the idle capacity in the system. For a mean utilization of 40\%, the average savings drop to 65\%, a  1.9$\times$ reduction when compared to our ideal case. 
}
\end{visionbox}

\vspace{-0.3cm}
\subsection{Savings with Latency Constrains}
\label{subsec:spatial-latency-constrained}
Apart from the capacity constraints, spatial migration could also be restricted by performance constraints such as response time. An ideal workload for spatial migration is the interactive requests originating from web-based services or inference-serving AI/ML systems. These workloads typically do not have any data dependency, and thus, their requests can be processed at any location in the world as long as the user receives the response to the request within a certain time frame. If a request can afford additional latency, it can potentially run at a greener datacenter if it can be reached within that period. As a result, there is a trade-off between the carbon savings and the increase in latency for such interactive workloads. Figure~\ref{fig:latency-and-smart-migration}(a) shows the average carbon savings, compared to average global carbon intensity, as a function of latency SLOs. We use the actual latency data for GCP that provides average latency information between two cloud endpoints within GCP~\cite{gcp_latency}. In each region, the average savings increase as the latency limit increases since requests can be routed to greener regions that might be further away. From the figure, it can be seen that most of the groupings, except Americas and Europe, require at least 200ms to achieve 90\% carbon savings. Americas and Europe need lower latency to achieve 90\% since the regions in this grouping are closer to the green regions as compared to Asia and Oceania. As the latency target increases to 300ms, all the regions in the world become accessible, which enables very high carbon savings. 
\vspace{-0.2cm}
\begin{visionbox}{}

\noindent\emph{\textbf{Key Takeaway.} When practical latency constraints are added to capacity constraints,
the savings from spatial shifting decrease further, with average savings dropping to 25\% for a 50ms latency constraint and 50\% datacenter utilization. }
\end{visionbox}
% \begin{figure}[t]
%     \begin{minipage}{0.5\linewidth}
%         \includegraphics[width=\linewidth]{figures/spatial/cap_gcp_latency.pdf}
%         % \vspace{0.5cm}
%         \subcaption{Capacity-Latency Constraints}
%     \end{minipage}\hfill
%     \begin{minipage}{0.5\linewidth}
%         \includegraphics[width=\linewidth]{figures/spatial/migrate_geo_lowest.pdf}
%         \subcaption{Smart Migration}
%     \end{minipage}
%     \vspace{-0.4cm}
%     \caption{\emph{Savings with Capacity and Latency constraints for region hopping and smart migration to the lowest within its own geographical grouping.}}   
%     \vspace{-0.6 cm}
%     \label{fig:latency-and-smart-migration}
% \end{figure}

\begin{figure}[t]
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/spatial/latency/cap_gcp_latency.pdf}
        % \vspace{0.5cm}
        \subcaption{Capacity-Latency}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/spatial/one-and-inf/migrate_geo_lowest.pdf}
        \subcaption{Smart Migration}
    \end{minipage}
    \vspace{-0.4cm}
    \caption{\emph{Savings with Capacity and Latency constraints for region hopping and smart migration to the lowest within its own geographical grouping.}}  
    \vspace{-0.8cm}
    \label{fig:latency-and-smart-migration}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{tabular}{ccc}
%         \includegraphics[width=0.5\linewidth]{figures/spatial/gcp_latency.pdf} & 
%     \includegraphics[width=0.5\linewidth]{figures/spatial/migrate_geo_lowest.pdf} \\
%     % \includegraphics[width=0.33\linewidth]{figures/imc_figures/spatial/heatmap/Global.pdf} \\
%     (a) Latency Constraint &  (b) Smart Migration
%     \end{tabular}
%     % \vspace{-0.4cm}
%     \caption{\emph{Latency for region hopping and smart migration to the lowest within grouping}}   
%     \vspace{-0.4cm}
%     \label{fig:latency-and-smart-migration}
% \end{figure}
% \begin{figure*}[!t]
%     \centering
%     \begin{tabular}{ccc}
%         \includegraphics[width=0.33\linewidth]{figures/spatial/gcp_latency.pdf} & 
%     \includegraphics[width=0.33\linewidth]{figures/spatial/migrate_geo_lowest.pdf} \\
%     % \includegraphics[width=0.33\linewidth]{figures/imc_figures/spatial/heatmap/Global.pdf} \\
%     (a) Latency Constraint &  (b) Smart Migration & (c) Heatmap
%     \end{tabular}
%     \vspace{-0.4cm}
%     \caption{\emph{Latency for region hopping and smart migration to the lowest within grouping}}   
%     \vspace{-0.6cm}
%     \label{fig:latency-and-smart-migration}
% \end{figure*}


% \vspace{-0.4 cm}
\subsection{Smart Region-hopping Policies}
\label{subsec:policies}
% infinite and one migration

To this point, our default spatial shifting policy has been to migrate once to the greenest available region. We chose this policy because it enables a simple spatial shifting policy based on historical averages which do not vary significantly on a per-year basis. However, as we discussed in \S\ref{sec:introduction}, there is an assumption that the carbon intensity patterns of various regions vary daily and weekly and thus may overlap or cross. In this case, a more sophisticated migration policy that hops between locations may yield more carbon savings than a simple one-time migration policy. To evaluate this hypothesis, we devise another spatial region-hopping policy that is clairvoyant, does not incur energy overhead to migrate, and immediately shifts to the destination. We refer to this policy as $\infty$-migrations, since it can migrate an infinite number of times, as compared to the 1-migration policy we have used so far. While we have been exploring spatial migration to the greenest region \emph{globally}, we want to constrain the migration to be within their geographical grouping in this experiment. This is to abstract out the \emph{global} lowest and any strict rankings for all the global traces. 

%\tammy{the explanation why we want to do geographical lowest instead of global lowest can be better.}

The results in Figure \ref{fig:latency-and-smart-migration}(b) show that carbon savings for both policies are relatively similar, with $\infty$-migration yielding only slightly higher savings but the difference between them being $<$1\%.  Thus, migrating once to the greenest region yields the vast majority of the savings, and more sophisticated migration approaches that migrate more often are unnecessary. Notably, our $\infty$-migration represents a best-case policy, as it ignores the overhead of migration. Thus, any practical policy outperforming 1-migration would have a very tight upper bound on its savings. In our current electric grid, this upper bound is less than 1\%. As a result, there are no practical benefits to sophisticated migration policies.
\vspace{-0.1cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaway.} A single migration to the greenest cloud region offers the majority of the benefits associated with spatial shifting. Even a clairvoyant policy that disregards the migration overhead adds, at most,  2\% additional carbon savings compared to the single migration policy.}
\end{visionbox}
%\noindent\emph{\textbf{Key Takeaway.} In today's world, migrating once to the greenest region gives most of the benefits of spatial shifting. Even a clairvoyant policy that ignores the overhead of migration yields at most 2\% more carbon savings than 1-migration.}

\subsection{Summary and System Implications}
\label{subsec:spatial_summary}

%Datacenters usually aim for nearly 0\% idle capacity and full utilization, which enables them to accommodate more workloads and effectively amortize their costs. 
%Many hyperscale datacenters maintain a PUE close to 1, indicating that they have optimized their cooling efficiency to the fullest extent. 
Our findings reveal a significant correlation between idle capacity and the benefits of spatial shifting: for every 1\% increase in global idle capacity, there is a corresponding $\sim$1\% reduction in global average emissions, equivalent to around 3.68 \emissionunit. 
%Notably, regions with high carbon intensity, particularly in Asia, experience substantial advantages when transitioning to greener locations. 
Nevertheless, this ultimately results in increased idleness in high intensity regions, and in over-provisioning in low intensity ones, which could have adverse implications on datacenters embodied carbon costs, primarily due to sub-optimal utilization of resources. 
%However, this ultimately results in increased idleness in high and over provisoning, which could have negative implications for datacenters embodied carbon costs, mainly due to even non-optimal utilization of resources. 
In addition, from a stability standpoint -- a factor that could potentially drive cloud customers to seek alternative solutions --, most datacenters need to operate at low capacity limits~\cite{huang2022metastable}.
This suggests datacenter regions should focus on optimizing their idle efficiency holistically, which could involve intelligent provision of servers to lower per-server load and accommodate more workloads, particularly relevant for low-intensity regions.
In contrast, high intensity regions can reduce their emissions through energy efficiency, for instance, with measures like DVFS that curtail energy consumption in response to workload intensity.
Additionally, spatial migration over shorter distances through e.g., edge computing, may prove more advantageous than relying on cloud resources because it can better exploit local renewable availability.
%These measures would enable cloud operators to not only better accommodate their workloads, it would also effectively amortize their overall costs. 

==> 6-camera-ready-temporal.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{tabular}{cc}
%     \includegraphics[width=0.49\linewidth]{figures/temporal/defer_slack_inf.pdf} & 
%     \includegraphics[width=0.49\linewidth]{figures/temporal/defer_slack_24.pdf} \\
%     % \includegraphics[width=0.21\linewidth]{figures/trace_grouped_boxplot/two_regions_grouped_boxplot.pdf} \\
%     (a) One-year slack &  (b) 24H slack 
%     \end{tabular}
%     \vspace{-0.4cm}
%     \caption{\emph{Average Defer Gains with respect to the global average }}   
%     % \vspace{-0.6cm}
%     \label{fig:temporal-defer}
% \end{figure}
\begin{figure}[t]
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/defer/defer_slack_8760.pdf}
        % \vspace{0.5cm}
        \subcaption{One-year slack}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/defer/defer_slack_24.pdf}
        \subcaption{24H slack}
    \end{minipage}
    \vspace{-0.4cm}
    \caption{\emph{Average Gains from Deferrability, with respect to the global average}}  
    \vspace{-0.4 cm}
    \label{fig:temporal-defer}
\end{figure}

In this section, we quantify the theoretical limits of temporal workload shifting by considering a scenario where workloads have a perfect knowledge of the future carbon intensity for the whole year. We call this case a one-year slack case. 
With this level of flexibility, a specific job can choose the most favorable time slot to start execution, thereby achieving the lowest carbon emissions in a region. We then analyze the carbon savings for different but limited levels of slack.
%With this very large slack, a given job can pick the time slots that will result in the region's lowest carbon emissions. We then analyze the carbon savings for different choices of slack. 
Next, we explore the effects of deferrability, interruptibility, as well as deferrability with interruptibilty, combined for both one-year slack and practical cases (see Section \ref{sec:background}). 
In practical scenarios, we opt for a 24-hour slack period, as it provides a sufficiently generous buffer within real-world settings~\cite{pradeep:sc20}.
%Note that for a practical scenario, we select the slack of 24 hours, for it is reasonably ample slack in a practical setting~\cite{pradeep:sc20}.

\subsection{Effects of Deferrability and Interruptibility}

\subsubsection*{\textbf{Deferrability}}
\label{subsec:deferrability}
% job length, fixed slack

%So far, the temporal analysis has been the average carbon savings for all job lengths mentioned in \S\ref{sec:methodology}, and that all jobs have the maximum degree of temporal flexibility (i.e., can be suspended and resumed). However, some jobs can only be deferred but, once started, cannot be interrupted. Moreover, different job lengths may have different degrees of temporal flexibility. Therefore, we want to analyze the upper bounds for carbon savings for different job lengths, where all the jobs are deferrable and non-interruptible. 

In this analysis, we examine the carbon savings from deferrability for both one-year and 24-hour slack settings. The carbon savings are relative to a non-deferrable job of the same length running in the same region. The datapoints are averages across all start times over a year. Figure \ref{fig:temporal-defer}(a) shows the theoretical upper bound of carbon savings from deferrability for each job length. From the figure, it can be seen that global carbon savings decrease from 41.8\% to 19.0\% as the job length increases from 1 hour to 168 hours. This is because as the job length increases, the job has to start occupying the “peaks” in the carbon trace despite being given the slack, while jobs that are <24 hours can utilize the slack to find the lowest valleys in the carbon trace. In a practical scenario, Figure \ref{fig:temporal-defer}(b) shows that the global carbon savings decrease from 15.4\% to 0.75\%. This is due to the relatively low fixed slack duration (24h) in comparison to the job lengths. For example, a 168-hour job with a 24-hour slack will have few opportunities to find periods with low carbon intensity compared to smaller jobs.

% \begin{figure}[t]
%     \centering
%     \begin{tabular}{cc}
%     \includegraphics[width=0.49\linewidth]{figures/temporal/interrupt_slack_inf.pdf} &
%     % \hspace{1em}
%     \includegraphics[width=0.49\linewidth]{figures/temporal/interrupt_slack_24.pdf} \\
%     % \hspace{2 cm}
%     % \includegraphics[width=0.21\linewidth]{figures/trace_grouped_boxplot/two_regions_grouped_boxplot.pdf} \\
%     (a) One-year slack &  (b) 24H slack 
%     \end{tabular}
%     \vspace{-0.4cm}
%     \caption{\emph{Average Interrupt Gains with respect to the global average}}   
%     % \vspace{-0.6cm}
%     \label{fig:temporal-interrupt}
% \end{figure}

\begin{figure}[t]
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/interrupt/interrupt_slack_8760.pdf}
        % \vspace{0.5cm}
        \subcaption{One-year slack}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/interrupt/interrupt_slack_24.pdf}
        \subcaption{24H slack}
    \end{minipage}
    \vspace{-0.4cm}
    \caption{\emph{Average Gains from Interruptibility, with respect to the global average}}  
    \vspace{-0.5 cm}
    \label{fig:temporal-interrupt}
\end{figure}

\subsubsection*{Interuptibility}
\label{subsec:interuptibility}
% job length, fixed slack

In addition to deferring a job’s start time, the ability to interrupt an already running job when energy’s carbon intensity increases is another dimension of temporal flexibility. Interruptibility enables schedulers to pause jobs when energy’s carbon intensity is high and resume them when it is low. Figure \ref{fig:temporal-interrupt}(a) shows the theoretical upper bound of additional carbon savings from interruptibility for each job length if they are interruptible and deferrable. Here, the global carbon savings from interruptibility increases from 0\% to 11\% as the job length increases. The carbon savings from interruptibility is at 0\% for a 1-hour job because the smallest granularity of a batch job in our setup is 1 hour, so it cannot be interrupted. Besides a 1-hour job, carbon savings from interruptibility increases mainly because long jobs can now be broken down into smaller jobs and run in low-carbon time slots throughout the year. While long jobs can exploit the effect of interruptibilty in an ideal case Figure \ref{fig:temporal-interrupt}(b) shows that the carbon savings reaches its peak at 24-hour job lengths at 5.1\% and gradually decreases as the job length increases. The 24-hour jobs exhibit the highest carbon savings because the 24-hour slack aligns with the job’s length, allowing the interruptibility policy to select very low-intensity periods from two carbon intensity “valleys” within the available 48-hour time window. Smaller jobs, however, gain lower carbon savings as most potential savings are gained simply by deferring them. Jobs longer than 24 hours also gain lower carbon savings as they need to occupy some “peaks” in the carbon trace even when interruptible. 


% \tammy{what should we name for the one-year slack case? I call this an infinite slack case because the experiment used 2022 and the infinite slack case is allow to look ahead for the whole year.}
% \begin{figure}[t]
%     \centering
%     \begin{tabular}{cc}
%         \includegraphics[width=0.49\linewidth]{figures/temporal/upperbound_global_pct_avg_equal_weigths_inf.pdf} & 
%     \includegraphics[width=0.49\linewidth]{figures/temporal/min_to_inf_slack.pdf} \\
%     % \includegraphics[width=0.21\linewidth]{figures/trace_grouped_boxplot/two_regions_grouped_boxplot.pdf} \\
%     (a) One-year slack &  (b) Slack and Savings 
%     \end{tabular}
%     \vspace{-0.4cm}
%     \caption{\emph{Infinite slack case and different choices of slack. The percentage is calculated by averaging all job lengths.}}  
%     % \vspace{-0.6cm}
%     \label{fig:temporal-meta}
% \end{figure}
% \tammy{Missing y label in (a) as Global Carbon Savings}

% \begin{figure}[t]
%     \centering
%     \begin{tabular}{cc}
%     \includegraphics[width=0.49\linewidth]{figures/temporal/stacked_slack_inf.pdf} & 
%     \includegraphics[width=0.49\linewidth]{figures/temporal/stacked_slack_24.pdf} \\
%     % \includegraphics[width=0.21\linewidth]{figures/trace_grouped_boxplot/two_regions_grouped_boxplot.pdf} \\
%     (a) Infinite (one-year) slack &  (b) 24H slack 
%     \end{tabular}
%     \vspace{-0.4cm}
%     \caption{\emph{Deferrability and Interruptibility gains, average with all job lengths from all regions}}   
%     % \vspace{-0.6cm}
%     \label{fig:temporal-defer-interrupt-stacked}
% \end{figure}

\begin{figure}[t]
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/defer-interrupt-combined/combined_savings_slack_8760.pdf}
        % \vspace{0.5cm}
        \subcaption{One-year slack}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/defer-interrupt-combined/combined_savings_slack_24.pdf}
        \subcaption{24H slack}
    \end{minipage}
    \vspace{-0.4cm}
    \caption{\emph{Average Gains from Deferrability and Interruptibility across all job lengths from all regions, with respect to the global average.}}  
    \vspace{-0.6 cm}
    \label{fig:temporal-defer-interrupt-stacked}
\end{figure}

\subsection*{Combined Deferrability and Interuptibility}
\label{subsec:deferrability_interuptibility}
% stacked bar graph

Figure \ref{fig:temporal-defer-interrupt-stacked} shows the breakdown of average carbon savings gained from deferrability and interruptibility across all regions. Figure \ref{fig:temporal-defer-interrupt-stacked}(a) shows that in the ideal setting, the benefits of deferrability decrease as the job length increases. However, interruptibility helps leverage carbon savings for long jobs. For 168-hour job, with just deferrability, the carbon saving is only at 19.0\%, but interruptibilty helps improve the carbon savings by another 11\%. In the practical scenario, however, even with interruptibility, the carbon savings remain small for long jobs. Figure \ref{fig:temporal-defer-interrupt-stacked}(b) shows that a 168-hour job only gains 11.8\% of carbon savings even if the job is deferrable and interruptible. This is because there are limited low-carbon regions for long jobs to run; hence, some parts of the job will run on a high-carbon period.

\vspace{-0.2cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaways. }
For temporal shifting, workloads benefit more from available slack and choice of start times than from the ability to be suspended and resumed.  However, the benefits of temporal shifting are far lower than those for spatial shifting,
with less than 19\% overall carbon savings for deferrable jobs with large slacks. }
%Jobs benefit more from deferrability than from interruptability, regardless of length. Deferrability leads to 19\% overall carbon savings, while short jobs yield the largest potential reductions and can achieve up to 55\% savings. Interruptability yields average carbon savings of no more than 12\%, even with large slacks.}
%Generally, the effectiveness of interruptability and temporal shifting hinges on slack being proportionate to job lengths, with the shortest jobs yielding the largest potential for savings.
\end{visionbox}

\begin{comment}
\vspace{-0.2cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaway (Deferrability with Interruptibility).} The carbon savings from interrupting a job's execution increase with job length, with large jobs seeing the greatest benefits. For any given job, the savings increase when slacks are larger than the job lengths. We find the average carbon savings across all jobs and all regions is less than 10\% even for large proportional slacks, with some jobs lengths and some regions seeing up to 12\% savings. Our results find that the overall efficacy of interruptability depends on the slack being proportional to job lengths.}
\end{visionbox}

\vspace{-0.2cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaway.} The carbon savings achieved by delaying the start time of a job diminish as its length increases, with the most substantial benefits observed for small jobs. Within a given job length, the savings increase proportionally with its slack. Our analysis reveals that, overall, global carbon deferrability savings reach 19\% for large slack values, with certain job lengths and specific regions achieving savings of up to 55\%. However, our results indicate that the overall effectiveness of temporal shifting will be constrained in the majority of regions for most job sizes, except for the smallest ones. \abel{will shorten it}}
\end{visionbox}
\end{comment}

%\subsection{Deferrability}
%\label{subsec:deferrability}

%Below, we quantify the benefits of temporal shifting globally for different workload mixes (\S\ref{subsec:temporal_starttime_def}) and different degrees of for deferring (\S\ref{subsec:deferrability})

\begin{figure*}[t]
    \begin{minipage}{0.24\linewidth}
         \includegraphics[width=\linewidth]{figs-eurosys24/temporal/weigthted_jobs/equal_slack_8760.pdf}
        % \vspace{0.5cm}
        \subcaption{Equally Distributed}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/weigthted_jobs/azure_slack_8760.pdf}
        % \vspace{0.5cm}
        \subcaption{Azure}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/weigthted_jobs/gcp_slack_8760.pdf}
        \subcaption{GCP}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs-eurosys24/temporal/vary-slack/vary_slack.pdf}
          % \vspace{-0.4cm}
        \subcaption{Vary Slack}
    \end{minipage}
    % \vspace{-0.4cm}
    % \caption{\emph{Deferrability and Interruptibility gains, with weighted average for all job lengths. Infinite slack case and different choices of slack. The percentage is calculated by averaging all job lengths.}}  
    \caption{\emph{Estimation of global and regional carbon reductions through the temporal shifting of workloads under different mixes of job lengths and datacenters with infinite slack, as well as global carbon savings for different choices of slacks}}  
    \vspace{-0.4 cm}
    \label{fig:temporal-real_trace}
\end{figure*}

\subsection{Effects of Slack}

\subsubsection*{Savings with One-Year Slack}
\label{subsec:temporal-inf-slack}


%Figure \ref{fig:temporal-meta}(a) 
Figure \ref{fig:temporal-real_trace}(a) shows the upper limit of temporal carbon savings for the one-year slack case. With a one-year slack, the average global temporal savings is 36.4\% with a variation of $\sim$24\%. By different geographical groupings, the average temporal carbon savings range from 16.6\% in Asia to 51.2\% in Oceania. Since Asia primarily relies on fossil fuels, it has a low variation of 13.5\%. On the contrary, Oceania has a higher percentage of renewables, hence more variations of 32.2\%, resulting in high carbon savings from temporal shifting. While using a one-year slack allows us to analyze the upper bound on ideal temporal shifting, the actual carbon savings are likely to be much, for the jobs are not willing to wait for an entire to run. We then next examine the effects of slack on cloud workloads.

\subsubsection*{Savings for Cloud Workloads}
\label{subsec:temporal-cloud}

%In the equal weighted workload mixes, the average savings is $\sim$15\%, while for 
Figure \ref{fig:temporal-real_trace}(b) and Figure \ref{fig:temporal-real_trace}(c) show the upper limit of cloud workload carbon savings for the one-year slack case.
While the average savings in the equally weighted workload is $\sim$38\%, in the Azure and Google traces, the average savings is $\sim$23\%.  The Azure and Google traces have a much higher percentage of long jobs ($>$48hrs), which, when combined with the large 10$\times$ slack and interruptibility, increase their flexibility to align with low carbon periods and increase their savings. In particular, in the Google trace, 1\% of the very long-running jobs ($>$1 week) account for 90\% of resource utilization and energy consumption~\cite{borg-next-gen}.  Thus, our analysis assumes that 90\% of the energy consumption can be delayed up to 10 weeks, which enables significant flexibility to align with low-carbon periods.  The carbon savings also increase as regions have more variations in their carbon intensity, which indicates higher fractions of solar and wind.  Since Asia mostly relies on fossil fuels, it has few variations and thus the carbon savings range from only 5-10\% across the workload mixes.  In contrast, Oceania has a higher percentage of renewables, more variations and more periodicity, which results in carbon savings ranging from 25-50\%.  Our analysis provides the upper bound on ideal temporal shifting.  Actual savings are likely to be much less due to less slack for long jobs, resource constraint that prevents running many jobs during low carbon periods, and uncertain carbon intensity forecasts.   We then next examine the effects of slack on temporal carbon savings.
%We next examine the impact of job length and slack on carbon savings when jobs are deferrable and interruptible. 

\subsubsection*{Savings with Varying Slacks}
\label{subsec:temporal-pratical-slack}
% slack graph
%Figure \ref{fig:temporal-meta}(b) 
Figure \ref{fig:temporal-real_trace}(d) shows temporal carbon savings for different slacks. With slack varying from 24 hours to one year, global carbon savings vary from 8.78\% to 36.4\%. This means that there is a large difference in temporal carbon savings between the ideal and practical setting. 
These findings suggest that temporal carbon savings exhibit sub-linear growth. Notably, beyond a 7-day timeframe, there are no substantial increases in savings observed in any of the regions.
%The results also imply that temporal carbon savings increase sub-linearly, and more importantly, after 7 days, no substantial gains in any of the regions is noted. 
% From 24 hours to one year, the slack increases by 365$\times$ while the carbon savings increase only by $\sim$76\%. 
From 24 hours to one year, the slack increases by 365$\times$ while the global carbon emissions decrease only by $\sim$38\%. 
This implies that harnessing carbon savings through temporal shifting in a real-world scheduling settings would require an exceptionally large amount of slack, an impractical proposition for most environments.
%This suggests that to leverage carbon savings from temporal shifting in a practical scenario based on scheduling, a very large slack is needed.

\vspace{-0.2cm}
\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaways. }
%Uniform datacenter workloads yield 38\% overall savings, even with large slacks. 
For real cloud workloads, savings from temporal shifting are limited to 23\%, and depend heavily upon factors like long job durations, substantial slack, absence of resource constraints, and access to future knowledge of carbon intensity.}
\end{visionbox}

\begin{comment}
\vspace{-0.2cm}
\begin{visionbox}{}
\noindent {\bf Key Takeaways (Slack)}. \emph{
	%The maximum potential global carbon savings from temporally shifting workloads is around 40\%. 
	Regions with higher reliance on renewable energy sources and greater fluctuations in their carbon intensity present significant potential for savings from temporally shifting. However, achieving savings in practice is limited, as they heavily rely on factors like long job durations, substantial slack, absence of resource constraints, and access to future knowledge of carbon intensity.}
\end{visionbox}
\end{comment}

\begin{comment}
\begin{figure}[t]
    %\begin{minipage}{0.5\linewidth}
    %     \includegraphics[width=\linewidth]{figures/temporal/upperbound_global_pct_avg_equal_weigths_inf.pdf}
        % \vspace{0.5cm}
    %    \subcaption{Infinite Slack}
    %\end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/temporal/min_to_inf_slack.pdf}
        \subcaption{Vary Slack}
    \end{minipage}
    \vspace{-0.4cm}
    \caption{\emph{Infinite slack case and different choices of slack. The percentage is calculated by averaging all job lengths.}}   
    \vspace{-0.6 cm}
    \label{fig:temporal-meta}
\end{figure}
\end{comment}

\subsection{Summary and System Implications}

Our findings highlight the importance of aligning job executions with periods of low carbon-intensity. 
However, the most substantial benefits of temporal shifting are enjoyed by small jobs, which decrease significantly as the duration of the workload approaches full daily cycles. 
Small jobs offer greater flexibility in determining their start times, and they can further leverage pause and resume techniques. 
That is, despite larger jobs typically having more slack, the only viable option for operators is to use suspend and resume techniques to align the execution of large jobs with low carbon-intensity periods.
When formulating carbon-efficient policies that use temporal shifting to enhance carbon efficiency, it is crucial to prioritize small jobs that can be scheduled during minimal valleys in a region's intensity trace. 
Additionally, contemporary workloads can be broken down into smaller interconnected processing components, effectively constituting a workflow of several smaller jobs that can benefit from temporal shifting. Therefore, leveraging this information has been explored in various studies, and integrating it into a carbon-aware orchestration, jointly with information from the local cloud or edge, is a viable approach to address the issue associated with long-running jobs.

%However, they also show that only small jobs get most of the benefits of temporal shifting. As we show, savings become negligible as the workload duration approaches whole daily cycles. 
%In contrast, small jobs posses various flexibility when beginning execution, and even more so when being able to use pause and resume techniques. 
%That is, even though a large job may usually have more slack, it still cannot benefit from savings as compared to smaller jobs.
%However, as savings become nonexistent the larger a job is, the only solution is for operators to interrupt jobs execution.
%Given a slack multiplier, the percentage savings of short job lengths ($< 24$h) are 2-3$\times$ higher than that of larger job lengths. This is because the length of a valley in the daily cycle of carbon intensity is large enough to fit jobs smaller than 24h. 
%When designing carbon efficient policies that use deferrability to improve carbon-efficiency, higher priority should be to schedule small jobs first because they can -- as opposed to large jobs that require large slacks -- be scheduled at minimal valleys throughout a region's intensity trace.
%Additionally, modern workloads have the flexibility to be broken down into different, smaller interlinked processing componenents, that together essentially form a workflow.
%Exploiting this information has been the subject of several work, and integrating it into an carbon-aware engine processing is a way to handle the issue with long running jobs.

==> 7-camera-ready-spatial_temporal.tex <==
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1.01\linewidth]{figs-eurosys24/temporal-spatial-combined/combined_savings_stacked.pdf}
% 	\vspace{-0.6cm}
% 	% \caption{}
% 	\caption[]{\emph{Breakdown of Spatial and Temporal Savings with the Net Gains for One-Year and 24H slacks. Flags indicate the destination regions where jobs from all regions migrate to.}}
% 	\label{fig:spatial_temporal_combined}
% 	\vspace{-0.5cm}
% \end{figure}

This section examines the combined effects of spatial and temporal shifting, quantifying their limits in ideal and practical settings. 
The approach allows jobs to not only migrate to different regions but also leverage deferrability to schedule their execution during optimal periods within the destination region. 
We consider two scenarios: the unconstrained case, where jobs can defer execution by up to a year, and the constrained case, where the deferral window is limited to 24 hours. 

\subsubsection*{Net Savings} Figure \ref{fig:spatial_temporal_combined} shows that, in general, regardless of the choice of slack, savings from spatial workload shifting dictate a decision on whether a workload should migrate to a particular region. That is, spatial savings dominate temporal savings regardless of its sign (positive, or negative). For example, migrating workloads to Sweden (SE), Ontario (CA-ON), or Belgium (BE) results in high net carbon savings because migrating to one of these regions yields high carbon savings from spatial shifting, even if these regions have low variability and therefore low temporal carbon savings. Conversely, migrating workloads to the Netherlands (NL), South Korea (KR), or Utah (US-UT) yields low to negative net gains in carbon savings (i.e. incurring more carbon emissions as compared to running the job locally) even when these regions have high temporal savings. This is because these regions have negative gains in carbon savings from spatial migration. Of course, there are some exceptions where regions have low spatial gains and high temporal gains and yet result in relatively high net carbon savings, such as California (US-CA) and Virginia (US-VA). However, in general, savings from spatial migration when migrating to a region influence the net gains in carbon savings.

% because these regions allow workloads to acquire high carbon savings from spatial migration. Conversely, migrating workloads to the Netherlands (NL), Virginia (US-VA), or South Korea (KR) yields low to negative net gains in carbon savings (i.e incurring more carbon emissions as compared to running the job locally) even when spatially migrating to this region has to 

% because there is a negative gain in carbon savings from spatial migration. 

% In an ideal case of one-year slack, Figure \ref{fig:spatial_temporal_combined} shows that 

%Through this analysis, we assess the independent impacts of spatial and temporal migration on carbon emissions to determine if temporal shifting can yield additional savings when combined with spatial shifting and whether the two approaches exhibit additive effects.

\begin{comment}
Finally, in this section we quantify the ideal and practical limits of spatial and temporal shifting when used in combination.
With this hybrid flexibility, a job can migrate to a region and in addition, use deferrability to schedule its execution to the best period within the destinated region to start execution.
We analyze two cases that compromise the ideal and practical cases. Although jobs can spatially migrate anywhere around the world in both cases, in the first unconstrained setting, jobs can defer execution by a year, and in the second constrained setting, by 24 hours.
We then quantify and compare the isolated effects that both spatial and temporal migration technique has on the carbon emissions. 
These cases serve to evaluate whether temporal shifting can add savings on top of the spatial shifting, and whether the two are additive.
%, i.e., is $Spatiotemporal_{savings} = Spatial_{savings} + Temporal_{savings}$?
\end{comment}

% \vspace{-0.2cm}

\begin{visionbox}{}
\noindent\emph{\textbf{Key Takeaways. } When combining spatial and temporal shifting, savings from spatial migration dominate the overall savings, with limited additional benefits from performing temporal shifting.
%In practice,  the net-effect from regions with significant potential savings from spatial shifting tend to outweigh the effect of potential temporal savings from other regions. Consequently, the decision of whether to spatially migrate to a region is mainly determined by the dominance of its spatial potential savings.
}

\end{visionbox}

